Dissecting Ponzi schemes on Ethereum: identification, analysis, and impact

Ponzi schemes are financial frauds which lure users under the promise of high profits. Actually, users are repaid only with the investments of new users joining the scheme: consequently, a Ponzi scheme implodes soon after users stop joining it. Originated in the offline world 150 years ago, Ponzi schemes have since then migrated to the digital world, approaching first the Web, and more recently hanging over cryptocurrencies like Bitcoin. Smart contract platforms like Ethereum have provided a new opportunity for scammers, who have now the possibility of creating "trustworthy" frauds that still make users lose money, but at least are guaranteed to execute "correctly". We present a comprehensive survey of Ponzi schemes on Ethereum, analysing their behaviour and their impact from various viewpoints.

==> ack.tex <==
\subsubsection*{Acknowledgments.} 

This work is partially supported by Aut.\ Reg.\ of Sardinia project P.I.A.\ 2013 ``NOMAD''.
%This work is partially funded by Aut.\ Reg.\ Sardinia under project NOMAD, % (Next generation Open Mobile Apps Development), 
%through P.I.A.\ 2013 -- Pacchetti Integrati di Agevolazione ``Industria Artigianato e Servizi''.

